3D CNN-based classification using sMRI and MD-DTI images for Alzheimer disease studies

Computer-aided early diagnosis of Alzheimers Disease (AD) and its prodromal form, Mild Cognitive Impairment (MCI), has been the subject of extensive research in recent years. Some recent studies have shown promising results in the AD and MCI determination using structural and functional Magnetic Resonance Imaging (sMRI, fMRI), Positron Emission Tomography (PET) and Diffusion Tensor Imaging (DTI) modalities. Furthermore, fusion of imaging modalities in a supervised machine learning framework has shown promising direction of research. In this paper we first review major trends in automatic classification methods such as feature extraction based methods as well as deep learning approaches in medical image analysis applied to the field of Alzheimer's Disease diagnostics. Then we propose our own algorithm for Alzheimer's Disease diagnostics based on a convolutional neural network and sMRI and DTI modalities fusion on hippocampal ROI using data from the Alzheimers Disease Neuroimaging Initiative (ADNI) database (http://adni.loni.usc.edu). Comparison with a single modality approach shows promising results. We also propose our own method of data augmentation for balancing classes of different size and analyze the impact of the ROI size on the classification results as well.

==> arxiv submission (2)/tables/architectures.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}configuration\\ name\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ convolutional\\ layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}convolution kernel\\ size for each layer\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ convolutional filters\\ in each layer\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of\\ fully-connected\\ layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number of units in\\  each fully-connected\\  layer\end{tabular}} \\ \hline
C1 & 4 & (5, 4, 3, 3) & (16, 32, 64, 128) & 2 & (16, 8) \\
C2 & 5 & (5, 4, 3, 3, 3) & (16, 32, 64, 128, 128) & 2 & (16, 8) \\
C3 & 5 & (7, 6, 5, 4, 3) & (16, 32, 64, 128, 256) & 2 & (32, 8) \\
C4 & 6 & (7, 6, 5, 4, 3, 3) & (16, 32, 64, 128, 256, 256) & 1 & 16 \\ \hline
\end{tabular}%
}
\caption{Compared architectures of the used neural networks}
\label{table:architectures}
\end{table*}


==> arxiv submission (2)/tables/comparison.tex <==
\begin{table*}[t]
\centering
\begin{footnotesize}
\begin{tabular}{|l|l|l|l|l|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Algorithm}} & \multicolumn{1}{c|}{\multirow{2}{*}{Methodology}} & \multicolumn{1}{c|}{\multirow{2}{*}{Modalities}} & \multicolumn{1}{c|}{\multirow{2}{*}{Content}} & \multicolumn{1}{c|}{\multirow{2}{*}{Data (size)}} & \multicolumn{3}{c|}{Accuracy}                                                          \\ \cline{6-8} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{AD/NC} & \multicolumn{1}{c|}{AD/MCI} & \multicolumn{1}{c|}{MCI/NC} \\ \hline

Magnin et al. \cite{volumetric:OBM} & Volumetric & sMRI & Full brain & custom (38) & 0.945 & - & - \\ \hline

Ahmed et al. \cite{f3_Jenny_pcc}  & Feature-based & sMRI & 2 ROIs & ADNI (509) & 0.838 & 0.695 & 0.621 \\ \hline
Ebadi et al. \cite{g1_graph_ensemble_2017} & Feature-based & DTI & Full brain & custom (34) & 0.8 & 0.833 & 0.7 \\ \hline
Lee et al. \cite{g3_svm_DTI_Korea} & Feature-based & DTI & Full brain & LONI (141) & 0.977 & 0.977 & - \\ \hline
Lei et al. \cite{g2_sift_China} & Feature-based & sMRI + PET & Full brain & ADNI (398) & 0.969 & - & 0.866 \\ \hline
Ahmed et al. \cite{f5_Jenny} & Feature-based & sMRI + DTI & 1 ROI & ADNI (203) & 0.902 & 0.766 & 0.794 \\ \hline

Vu et al. \cite{c4_sparse_encoder_Korea} & NN-based & sMRI + PET & Full brain & ADNI (203) & 0.91 & - & - \\ \hline
Payan and Montana \cite{c8_medical_UK} & NN-based & sMRI & Full brain & ADNI (2265) & 0.993 & 1 & 0.942 \\ \hline
Glozman and Liba \cite{c1_report_Standford} & NN-based & sMRI + PET & Full brain & ADNI (1370) & 0.665 & - & - \\ \hline
Sarraf et al. \cite{c7.1_DeepAd_Canada} & NN-based & sMRI, fMRI & Full brain & ADNI (302) & 0.988, 0.999 & - & - \\ \hline
Billones et al. \cite{c5_demnet_Philippines} & NN-based & sMRI & Full brain & ADNI (900) & 0.983 & 0.939 & 0.917 \\ \hline
Aderghal et al. \cite{Aderghal} & NN-based & sMRI & 1 ROI & ADNI (815) & 0.914 & 0.695 & 0.656 \\ \hline
Shi et al. \cite{c9_DPN_China} & NN-based & sMRI + PET & Full brain & ADNI (202) & 0.971 & - & 0.872 \\ \hline
Korolev et al. \cite{c3_Skolkovo} & NN-based & sMRI & Full brain & ADNI (231) & 0.79-0.8 & - & - \\ \hline
Suk et al. \cite{c6_deep_ensemble_sparse_regr_Korea} & NN-based & sMRI & 93 ROIs & ADNI (805) & 0.903 & - & 0.742 \\ \hline
Suk et al. \cite{c6_deep_ensemble_sparse_regr_Korea} & NN-based & sMRI & 93 ROIs & ADNI (805) & 0.903 & - & 0.742 \\ \hline
Luo et al. \cite{ex_2} & NN-based & sMRI & 7 ROIs & ADNI (81) & 0.83 & - & - \\ \hline
Wang et al. \cite{ex_3} & NN-based & sMRI & Full brain & ADNI (629) & - & - & 0.906 \\ \hline
Li et al. \cite{ex_5} & NN-based & sMRI & 1 ROI & ADNI (1776) & 0.965 & 0.67 & 0.622 \\ \hline
Cheng et al. \cite{ex_7} & NN-based & sMRI & 27 ROIs & ADNI (1428) & 0.872 & - & - \\ \hline
Li et al. \cite{ex_9} & NN-based & sMRI & Full brain & ADNI (832) & 0.91 & 0.877 & 0.855 \\ \hline


\end{tabular}
\end{footnotesize}
\label{comparison_table}
\caption{Comparison of different state of the art classification methods.}
\end{table*}


==> arxiv submission (2)/tables/demographic.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Diagnosis & Subjects & Age                                                                              & \begin{tabular}[c]{@{}c@{}}Gender\\ (F/M)\end{tabular} & MMSE               \\ \hline
AD        & 48       & \begin{tabular}[c]{@{}c@{}}{[}55.72 - 91.53{]}\\ 75.65 \(\pm\) 8.63\end{tabular} & 20 / 28                                                & 23.0 \(\pm\) 2.42  \\
MCI       & 108      & \begin{tabular}[c]{@{}c@{}}{[}55.32 - 91.88{]}\\ 73.46 \(\pm\) 7.47\end{tabular} & 42 / 66                                                & 27.39 \(\pm\) 1.99 \\
NC        & 58       & \begin{tabular}[c]{@{}c@{}}{[}60.40 - 89.59{]}\\ 73.41 \(\pm\) 5.90\end{tabular} & 30 / 28                                                & 28.88 \(\pm\) 1.18 \\ \hline
\end{tabular}%
}
\caption{Demographic description of the ADNI group, Values are denoted as intervals and as mean \(\pm\) std}
\label{table:demographic}
\end{table}

==> arxiv submission (2)/tables/results_AD_MCI.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
% \tabcolsep=0.11cm
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|ccc|ccc|ccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean ACC\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SEN\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SPC\\ {[}95\% CI{]}\end{tabular}}} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}used\\ data\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}ROI\\ size\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}configu-\\ ration\end{tabular}}} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} \\ \hline
 &  & C1 & \textbf{\begin{tabular}[c]{@{}c@{}}0.754\\ \(\pm\)0.172\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.760\\ \(\pm\)0.054\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.759\\ \(\pm\)0.054\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.617\\ \(\pm\)0.195\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.638\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.639\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.950\\ \(\pm\)0.069\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.962\\ \(\pm\)0.024\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.953\\ \(\pm\)0.027\end{tabular} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.746\\ \(\pm\)0.174\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.736\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.754\\ \(\pm\)0.054\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.600\\ \(\pm\)0.196\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.633\\ \(\pm\)0.061\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.609\\ \(\pm\)0.062\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.967\\ \(\pm\)0.053\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.959\\ \(\pm\)0.025\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.956\\ \(\pm\)0.026\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.642\\ \(\pm\)0.192\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.677\\ \(\pm\)0.059\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.663\\ \(\pm\)0.060\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.525\\ \(\pm\)0.200\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.565\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.526\\ \(\pm\)0.063\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}1.00\\ \(\pm\)0.000\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.982\\ \(\pm\)0.017\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.958\\ \(\pm\)0.025\end{tabular} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.679\\ \(\pm\)0.187\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.731\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.690\\ \(\pm\)0.059\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.658\\ \(\pm\)0.190\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.708\\ \(\pm\)0.058\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.711\\ \(\pm\)0.057\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.992\\ \(\pm\)0.022\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.999\\ \(\pm\)0.002\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.991\\ \(\pm\)0.011\end{tabular} \\
 &  & C3 & \begin{tabular}[c]{@{}c@{}}0.688\\ \(\pm\)0.185\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.651\\ \(\pm\)0.060\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.678\\ \(\pm\)0.059\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.592\\ \(\pm\)0.197\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.553\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.610\\ \(\pm\)0.062\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}1.000\\ \(\pm\)0.000\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.983\\ \(\pm\)0.017\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.978\\ \(\pm\)0.019\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.683\\ \(\pm\)0.186\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.708\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.717\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.433\\ \(\pm\)0.198\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.478\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.476\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.983\\ \(\pm\)0.034\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.983\\ \(\pm\)0.016\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.978\\ \(\pm\)0.018\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}0.717\\ \(\pm\)0.180\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.694\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.693\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.692\\ \(\pm\)0.185\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.597\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.644\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.992\\ \(\pm\)0.022\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.992\\ \(\pm\)0.010\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.973\\ \(\pm\)0.020\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.717\\ \(\pm\)0.180\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.709\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.704\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.575\\ \(\pm\)0.198\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.530\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.520\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}1.000\\ \(\pm\)0.000\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.997\\ \(\pm\)0.005\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.996\\ \(\pm\)0.006\end{tabular}} \\ \hline
 &  & C1 & \begin{tabular}[c]{@{}c@{}}0.725\\ \(\pm\)0.179\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.742\\ \(\pm\)0.055\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.736\\ \(\pm\)0.056\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.533\\ \(\pm\)0.200\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.597\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.569\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.958\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.954\\ \(\pm\)0.027\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.951\\ \(\pm\)0.027\end{tabular} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.783\\ \(\pm\)0.165\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.735\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.788\\ \(\pm\)0.052\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.867\\ \(\pm\)0.135\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.832\\ \(\pm\)0.047\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.865\\ \(\pm\)0.043\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.917\\ \(\pm\)0.097\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.863\\ \(\pm\)0.044\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.886\\ \(\pm\)0.040\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.7792\\ \(\pm\)0.166\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.767\\ \(\pm\)0.054\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.777\\ \(\pm\)0.053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.858\\ \(\pm\)0.140\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.863\\ \(\pm\)0.044\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.813\\ \(\pm\)0.049\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.908\\ \(\pm\)0.104\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.913\\ \(\pm\)0.036\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.909\\ \(\pm\)0.036\end{tabular} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\\ +\\ DTI\_L\\ +\\ DTI\_R\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.800\\ \(\pm\)0.213\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.751\\ \(\pm\)0.077\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.791\\ \(\pm\)0.073\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.933\\ \(\pm\)0.104\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.927\\ \(\pm\)0.047\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.902\\ \(\pm\)0.053\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.149\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.893\\ \(\pm\)0.055\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.875\\ \(\pm\)0.059\end{tabular} \\
 &  & C3 & \begin{tabular}[c]{@{}c@{}}0.738\\ \(\pm\)0.176\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.734\\ \(\pm\)0.056\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.763\\ \(\pm\)0.054\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.692\\ \(\pm\)0.185\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.708\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.723\\ \(\pm\)0.057\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.116\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.876\\ \(\pm\)0.042\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.903\\ \(\pm\)0.037\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.721\\ \(\pm\)0.180\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.743\\ \(\pm\)0.055\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.744\\ \(\pm\)0.055\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.650\\ \(\pm\)0.191\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.699\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.674\\ \(\pm\)0.059\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.900\\ \(\pm\)0.110\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.909\\ \(\pm\)0.036\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.914\\ \(\pm\)0.035\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}0.788\\ \(\pm\)0.164\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.787\\ \(\pm\)0.052\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.787\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.792\\ \(\pm\)0.163\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.771\\ \(\pm\)0.053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.778\\ \(\pm\)0.053\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.992\\ \(\pm\)0.022\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.985\\ \(\pm\)0.015\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.986\\ \(\pm\)0.015\end{tabular}} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.738\\ \(\pm\)0.176\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.734\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.739\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.625\\ \(\pm\)0.194\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.619\\ \(\pm\)0.061\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.623\\ \(\pm\)0.061\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.983\\ \(\pm\)0.034\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.978\\ \(\pm\)0.019\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.977\\ \(\pm\)0.019\end{tabular} \\ \hline
\end{tabular}%
}
\caption{AD-MCI classification results. Here \(\alpha \pm \beta\) designation corresponds to the top-mean value of metric and it's \(95\%\) confidence interval. \(\alpha\) - metric value, \([\alpha-\beta, \alpha+\beta]\) - confidence interval.}
\label{table:results_AD_MCI}
\end{table*}

==> arxiv submission (2)/tables/results_AD_NC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
% \tabcolsep=0.11cm
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|ccc|ccc|ccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean ACC\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SEN\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SPC\\ {[}95\% CI{]}\end{tabular}}} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}used\\ data\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}ROI\\ size\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}configu-\\ ration\end{tabular}}} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} \\ \hline
 &  & C1 & \textbf{\begin{tabular}[c]{@{}c@{}}0.854\\ \(\pm\) 0.141\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.827\\ \(\pm\) 0.048\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.839\\ \(\pm\) 0.047\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\) 0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.880\\ \(\pm\) 0.041\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\) 0.041\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.900\\ \(\pm\) 0.110\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}0.885\\ \(\pm\) 0.040\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.901\\ \(\pm\) 0.038\end{tabular}} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.825\\ \(\pm\)0.152\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.813\\ \(\pm\)0.049\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.813\\ \(\pm\)0.049\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.867\\ \(\pm\)0.135\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.848\\ \(\pm\)0.046\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.850\\ \(\pm\)0.045\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.908\\ \(\pm\)0.104\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.879\\ \(\pm\)0.0412\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.869\\ \(\pm\)0.043\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.808\\ \(\pm\)0.158\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.790\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.801\\ \(\pm\)0.051\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.775\\ \(\pm\)0.167\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.799\\ \(\pm\)0.051\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.786\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.831\\ \(\pm\)0.047\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.863\\ \(\pm\)0.044\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.767\\ \(\pm\)0.169\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.769\\ \(\pm\)0.053\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.776\\ \(\pm\)0.053\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.825\\ \(\pm\)0.152\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.809\\ \(\pm\)0.050\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.804\\ \(\pm\)0.050\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.817\\ \(\pm\)0.155\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.816\\ \(\pm\)0.049\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.828\\ \(\pm\)0.048\end{tabular} \\
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\end{tabular}} &  & C3 & \begin{tabular}[c]{@{}c@{}}0.800\\ \(\pm\)0.160\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.777\\ \(\pm\)0.053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.790\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.792\\ \(\pm\)0.163\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.813\\ \(\pm\)0.049\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.790\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.894\\ \(\pm\)0.039\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.882\\ \(\pm\)0.041\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.771\\ \(\pm\)0.168\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.725\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.757\\ \(\pm\)0.054\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.725\\ \(\pm\)0.179\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.711\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.724\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.116\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.821\\ \(\pm\)0.049\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.827\\ \(\pm\)0.048\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}0.788\\ \(\pm\)0.164\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.779\\ \(\pm\)0.053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.779\\ \(\pm\)0.053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.767\\ \(\pm\)0.169\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.742\\ \(\pm\)0.055\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.738\\ \(\pm\)0.056\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.864\\ \(\pm\)0.043\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.854\\ \(\pm\)0.045\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.842\\ \(\pm\)0.146\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.829\\ \(\pm\)0.048\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.836\\ \(\pm\)0.047\end{tabular} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.925\\ \(\pm\)0.090\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.888\\ \(\pm\)0.040\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.898\\ \(\pm\)0.038\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.858\\ \(\pm\)0.140\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.852\\ \(\pm\)0.045\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.838\\ \(\pm\)0.047\end{tabular} \\ \hline
 &  & C1 & \begin{tabular}[c]{@{}c@{}}0.875\\ \(\pm\) 0.129\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.874\\ \(\pm\) 0.042\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.854\\ \(\pm\)0.045\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.116\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.901\\ \(\pm\)0.038\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.874\\ \(\pm\)0.042\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.116\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.901\\ \(\pm\)0.038\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.887\\ \(\pm\)0.040\end{tabular} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.116\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.904\\ \(\pm\)0.037\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.885\\ \(\pm\)0.040\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.933\\ \(\pm\)0.083\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.940\\ \(\pm\)0.030\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.904\\ \(\pm\)0.037\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.917\\ \(\pm\)0.097\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.914\\ \(\pm\)0.035\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.912\\ \(\pm\)0.036\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.904\\ \(\pm\)0.037\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.891\\ \(\pm\)0.040\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.925\\ \(\pm\)0.090\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.923\\ \(\pm\)0.034\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.918\\ \(\pm\)0.035\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.123\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.910\\ \(\pm\)0.036\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.910\\ \(\pm\)0.036\end{tabular} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\\ +\\ DTI\_L\\ +\\ DTI\_R\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.842\\ \(\pm\)0.146\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.854\\ \(\pm\)0.045\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.842\\ \(\pm\)0.046\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.925\\ \(\pm\)0.090\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.873\\ \(\pm\)0.042\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.892\\ \(\pm\)0.039\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.875\\ \(\pm\)0.129\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.041\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.872\\ \(\pm\)0.042\end{tabular} \\
 &  & C3 & \begin{tabular}[c]{@{}c@{}}0.900\\ \(\pm\)0.110\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.908\\ \(\pm\)0.037\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.895\\ \(\pm\)0.039\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.933\\ \(\pm\)0.083\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.907\\ \(\pm\)0.037\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.910\\ \(\pm\)0.036\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.917\\ \(\pm\)0.097\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.924\\ \(\pm\)0.034\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.913\\ \(\pm\)0.036\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.908\\ \(\pm\)0.104\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.871\\ \(\pm\)0.042\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.866\\ \(\pm\)0.043\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.850\\ \(\pm\)0.143\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.823\\ \(\pm\)0.048\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.806\\ \(\pm\)0.050\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.992\\ \(\pm\)0.022\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.973\\ \(\pm\)0.021\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.956\\ \(\pm\)0.026\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}0.904\\ \(\pm\)0.107\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.903\\ \(\pm\)0.038\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.895\\ \(\pm\)0.039\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.867\\ \(\pm\)0.135\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.883\\ \(\pm\)0.041\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.871\\ \(\pm\)0.042\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.942\\ \(\pm\)0.076\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.923\\ \(\pm\)0.034\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.924\\ \(\pm\)0.034\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.967\\ \(\pm\) 0.055\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.938\\ \(\pm\) 0.03\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.947\\ \(\pm\) 0.03\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.958\\ \(\pm\) 0.06\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.943\\ \(\pm\) 0.03\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.936\\ \(\pm\) 0.035\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.975\\ \(\pm\) 0.06\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.939\\ \(\pm\) 0.03\end{tabular}} & \cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}0.964\\ \(\pm\) 0.035\end{tabular}} \\ \hline
\end{tabular}%
}\caption{AD-NC classification results. Here \(\alpha \pm \beta\) designation corresponds to the top-mean value of metric and it's \(95\%\) confidence interval. \(\alpha\) - metric value, \([\alpha-\beta, \alpha+\beta]\) - confidence interval.}
\label{table:results_AD_NC}
\end{table*}

==> arxiv submission (2)/tables/results_MCI_NC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
% \tabcolsep=0.11cm
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|ccc|ccc|ccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean ACC\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SEN\\ {[}95\% CI{]}\end{tabular}}} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Top-mean SPC\\ {[}95\% CI{]}\end{tabular}}} \\
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}used\\ data\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}ROI\\ size\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}configu-\\ ration\end{tabular}}} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} & \textbf{test 0} & \textbf{test 1} & \textbf{test 2} \\ \hline
 &  & C1 & \begin{tabular}[c]{@{}c@{}}0.588\\ \(\pm\)0.197\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.558\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.542\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.733\\ \(\pm\)0.177\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.710\\ \(\pm\)0.057\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.699\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.750\\ \(\pm\)0.173\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.725\\ \(\pm\)0.057\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.718\\ \(\pm\)0.057\end{tabular} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.571\\ \(\pm\)0.198\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.564\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.578\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.875}\\ \textbf{\(\pm\)0.129}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.832}\\ \textbf{\(\pm\)0.047}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.810}\\ \textbf{\(\pm\)0.050}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.558\\ \(\pm\)0.199\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.528\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.605\\ \(\pm\)0.062\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.608\\ \(\pm\)0.195\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.630\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.603\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.667\\ \(\pm\)0.189\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.643\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.667\\ \(\pm\)0.060\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.775\\ \(\pm\)0.167\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.759\\ \(\pm\)0.054\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.797\\ \(\pm\)0.051\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.571\\ \(\pm\)0.198\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.593\\ \(\pm\)0.062\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.593\\ \(\pm\)0.062\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.667\\ \(\pm\)0.189\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.674\\ \(\pm\)0.059\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.638\\ \(\pm\)0.061\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.575\\ \(\pm\)0.198\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.583\\ \(\pm\)0.062\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.600\\ \(\pm\)0.062\end{tabular} \\
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\end{tabular}} &  & C3 & \begin{tabular}[c]{@{}c@{}}0.642\\ \(\pm\)0.271\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.614\\ \(\pm\)0.087\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.602\\ \(\pm\)0.088\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.592\\ \(\pm\)0.278\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.608\\ \(\pm\)0.087\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.550\\ \(\pm\)0.089\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.733\\ \(\pm\)0.250\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.673\\ \(\pm\)0.084\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.735\\ \(\pm\)0.079\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.625\\ \(\pm\)0.194\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.631\\ \(\pm\)0.061\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.618\\ \(\pm\)0.062\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.783\\ \(\pm\)0.165\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.769\\ \(\pm\)0.053\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.748\\ \(\pm\)0.055\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.558\\ \(\pm\)0.199\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.525\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.553\\ \(\pm\)0.063\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}\textbf{0.658}\\ \textbf{\(\pm\)0.268}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.657}\\ \textbf{\(\pm\)0.085}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.631}\\ \textbf{\(\pm\)0.086}\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.800\\ \(\pm\)0.213\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.778\\ \(\pm\)0.074\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.713\\ \(\pm\)0.081\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.817}\\ \textbf{\(\pm\)0.201}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.788}\\ \textbf{\(\pm\)0.073}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.788}\\ \textbf{\(\pm\)0.073}\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.542\\ \(\pm\)0.199\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.502\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.518\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.683\\ \(\pm\)0.186\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.696\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.671\\ \(\pm\)0.060\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.600\\ \(\pm\)0.196\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.560\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.618\\ \(\pm\)0.062\end{tabular} \\ \hline
 &  & C1 & \begin{tabular}[c]{@{}c@{}}0.538\\ \(\pm\)0.200\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.532\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.517\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.767\\ \(\pm\)0.169\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.788\\ \(\pm\)0.052\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.693\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.500\\ \(\pm\)0.200\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.518\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.542\\ \(\pm\)0.063\end{tabular} \\
 & \multirow{-2}{*}{28} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.538\\ \(\pm\)0.200\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.563\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.548\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.800\\ \(\pm\)0.160\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.777\\ \(\pm\)0.053\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.713\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.500\\ \(\pm\)0.200\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.472\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.504\\ \(\pm\)0.063\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C1 & \begin{tabular}[c]{@{}c@{}}0.542\\ \(\pm\)0.199\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.547\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.556\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.758\\ \(\pm\)0.171\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.738\\ \(\pm\)0.056\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.706\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.417\\ \(\pm\)0.197\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.403\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.501\\ \(\pm\)0.063\end{tabular} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}sMRI\_L\\ +\\ sMRI\_R\\ +\\ DTI\_L\\ +\\ DTI\_R\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}38} & \cellcolor[HTML]{EFEFEF}C2 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.625}\\ \textbf{\(\pm\)0.194}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.613}\\ \textbf{\(\pm\)0.062}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.612}\\ \textbf{\(\pm\)0.062}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.858}\\ \textbf{\(\pm\)0.140}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.834}\\ \textbf{\(\pm\)0.047}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}\textbf{0.792}\\ \textbf{\(\pm\)0.051}\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.458\\ \(\pm\)0.199\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.441\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.520\\ \(\pm\)0.063\end{tabular} \\
 &  & C3 & \begin{tabular}[c]{@{}c@{}}0.621\\ \(\pm\)0.194\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.628\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.608\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.708\\ \(\pm\)0.182\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.759\\ \(\pm\)0.054\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.690\\ \(\pm\)0.059\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.600}\\ \textbf{\(\pm\)0.196}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.570}\\ \textbf{\(\pm\)0.063}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{0.624}\\ \textbf{\(\pm\)0.061}\end{tabular} \\
 & \multirow{-2}{*}{42} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.513\\ \(\pm\)0.200\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.537\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.531\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.692\\ \(\pm\)0.185\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.728\\ \(\pm\)0.056\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.673\\ \(\pm\)0.060\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.408\\ \(\pm\)0.197\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.424\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.453\\ \(\pm\)0.063\end{tabular} \\
 & \cellcolor[HTML]{EFEFEF} & C3 & \begin{tabular}[c]{@{}c@{}}0.588\\ \(\pm\)0.197\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.585\\ \(\pm\)0.062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.573\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.708\\ \(\pm\)0.182\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.697\\ \(\pm\)0.058\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.638\\ \(\pm\)0.061\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.567\\ \(\pm\)0.198\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.520\\ \(\pm\)0.063\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.604\\ \(\pm\)0.062\end{tabular} \\
 & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}48} & \cellcolor[HTML]{EFEFEF}C4 & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.554\\ \(\pm\)0.199\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.543\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.552\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.725\\ \(\pm\)0.179\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.719\\ \(\pm\)0.057\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.707\\ \(\pm\)0.058\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.467\\ \(\pm\)0.200\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.450\\ \(\pm\)0.063\end{tabular} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}0.471\\ \(\pm\)0.063\end{tabular} \\ \hline
\end{tabular}%
}
\caption{MCI-NC classification results. Here \(\alpha \pm \beta\) designation corresponds to the top-mean value of metric and it's \(95\%\) confidence interval. \(\alpha\) - metric value, \([\alpha-\beta, \alpha+\beta]\) - confidence interval.}
\label{table:results_MCI_NC}
\end{table*}
